A Finite-Gain Stability Approach to NMPC Design: the Extended Version

This paper proposes a novel approach to design of Nonlinear Model Predictive Control (NMPC) schemes based on Finite-Gain Stability (FGS) concepts. The proposed formulation considers the case where the plant is affected by unknown but bounded disturbances, which renders difficult the classical Lyapunov-based analysis/design. Based on FGS conditions for a closed-loop system, we develop a systematic NMPC design methodology, allowing us to choose the relevant NMPC parameters that lead to closed-loop FGS and provide a satisfactory tracking performance, also for the case of time-varying reference signals. A simulated example is presented to demonstrate the effectiveness of our framework, concerned with lateral/longitudinal control of an automated vehicle.

==> nmpc_design_1.tex <==

\section{NMPC design} \label{sec:nmpc_des}
This section presents a systematic methodology for the selection of a suitable NMPC configuration giving closed-loop finite-gain stability, as defined by Theorem \ref{th:fgs_dist}, while providing satisfactory tracking performance. The design procedure consists of three key steps: (i) determination of the integer horizon $\tau$ used in the finite-gain analysis; (ii) a Monte Carlo campaign that generates candidate NMPC configurations and closed-loop data over a finite interval of length $\tau$; (iii) a selection rule that chooses the best configuration according to both tracking error and stability criteria.

Let $\Phi$ denote a finite set of NMPC configurations. Each configuration $\phi\in\Phi$ is described by a prediction horizon $T_p$ and weighting matrices $R,Q,P \succ 0$. Let $s=(x_0,r)$ be a generic scenario containing an initial state $x_0\in\mathcal{X}_0$ and a reference sequence $r=(r_{0},r_{1},\dots)\in\mathcal{R}$.

At a given time $t$ and for a fixed configuration $\phi$ and scenario $s$, denote: i) $x_t(\phi,s)$  the closed-loop state trajectory produced by the NMPC law; ii) $e_t(\phi,s)$ the corresponding tracking error; and iii) $F_t^{\tau}(\phi,s)$ the transition matrix. 
Finally, denote by $\lambda_{\max}(\cdot)$ the spectral radius, i.e., the largest eigenvalue magnitude, of a given matrix.

In the following, the design methodology is described in detail.

\subsection{Selection of the simulation horizon $\tau$}
The integer $\tau$, introduced in Assumption \ref{ass:assumption_FGS}-A3 and Theorem \ref{th:fgs_dist}, must be chosen sufficiently large to ensure that the spectral radius of the product $F^{\tau}_t(\phi,s)$ remains strictly less than one for all the considered scenarios. We propose the following procedure:


\begin{enumerate}
  \item Generate an initial scenario set $\mathcal{S}_{\mathrm{in}}=\{s^1,\dots,s^M\}$, where each element is defined as $s^i=(x^i_0,r^i)$.
  \item Choose a nominal NMPC configuration $\phi_{\mathrm{nom}}$ (e.g. obtained from design heuristics such as Bryson's rule).
  \item For $\tau=1,2,\dots$ and for each scenario $s^i \in \mathcal{S}_{\mathrm{in}}$ compute $\gamma$.
  % \[
  %   \kappa^i_t(\tau) = \lambda_{\max}\big(F^{\tau,i}_t(\phi_{\mathrm{nom}},s^i)\big).
  % \]
  \item Select the smallest integer $\tau^\star$ such that
  \begin{equation}\label{eq:tau_choice}
    \sup_{i\in\{1,\dots,M\}}\;\gamma<\;1.
  \end{equation}
\end{enumerate}

If~\eqref{eq:tau_choice} cannot be satisfied for any $\tau$, it may be necessary to modify $\phi_{\mathrm{nom}}$ (e.g. increase $T_p$ or retune $Q,R,P$) or relax performance requirements.

\subsection{Monte Carlo campaign}
A Monte Carlo campaign is conducted to evaluate the finite-time closed-loop response for each NMPC configuration. The steps are:


\begin{enumerate}
  \item Generate an evaluation scenario set $\mathcal{S}=\{s^1,\dots,s^N\}$, with $N \ge M$. This set is typically constructed in order to ensure a proper coverage of the relevant initial states and reference trajectories, and may be an an extension of the initial scenario set, i.e., $\mathcal{S}\supseteq\mathcal{S}_{\mathrm{in}}$. 
  \item Build the NMPC configuration set
  \[
    \Phi=\{\phi_j\}_{j=1}^K,\qquad \phi_j=(T_p^{(j)},Q^{(j)},R^{(j)},P^{(j}),
  \]
  by choosing different values of $T_p$, $Q,R$ and $P$. The matrices $Q$ and $R$ can be initialized using Bryson’s rule,
  \begin{equation}\label{eq:bryson}
    Q_0=\operatorname{diag}(1/x_{max}^2),\quad
    R_0=\operatorname{diag}(1/u_{max}^2),
  \end{equation}
  where $x_{max}$ and $u_{max}$ are the maximum values for the state and input components, respectively.  The set of $Q$ and $R$ are then generated through variations about $Q_0$ and $R_0$ 
  \[
  Q=\alpha_Q Q_0,
  \]
  \[
  R=\alpha_R R_0,
  \]
where $\alpha_Q,\alpha_R>0$ are scalar tuning parameters.
  \item For each $(\phi_j,s^i)$, simulate the closed-loop state trajectory $x_t(\phi,s^i)$ over the time interval $t=1,\dots,\tau^\star$ and store the resulting tracking error $e_{\tau^\star}(\phi_j,s^i)$ and transition matrix $F^{\tau^\star}_t(\phi_j,s^i)$.
\end{enumerate}

\subsection{Performance metrics and selection rule}
For each NMPC configuation $\phi \in \Phi$, we define two metrics:

\paragraph{Tracking error metric}
The worst-case tracking error over all scenarios is defined as
\begin{equation}\label{eq:E_c}
E(\phi)=\max_{i=1,\dots,N} E(\phi,s^i)=\max_{i=1,\dots,N}\|e_{\tau^\star}(\phi,s^i)\|_2.
\end{equation}


\paragraph{Finite-gain stability metric}
The worst-case finite-gain stability index is given by
\begin{equation}\label{eq:L_c}
L(\phi)=\max_{i=1,\dots,N}\lambda_{\max}\big(F^{\tau^\star}_t(\phi,s^i)\big).
\end{equation}


For the selection rule, we first normalize the two metrics relative to their worst-case values across the entire set $\Phi$
\[
    E_n(\phi)=\frac{E(\phi)}{\max_{\Phi}E},\qquad
    L_n(\phi)=\frac{L(\phi)}{\max_{\Phi}L},
  \]
and then define the following cost function 
  \begin{equation}
    J_{sr}(\phi)=\alpha_J E_n(\phi)+(1-\alpha_J) L_n(\phi),\qquad \alpha_J\in[0,1].
  \end{equation}
  Finally, the optimal NMPC configuration is selected as
  \begin{equation}\label{eq:Jc}
  \phi^\star=\arg\min_{\phi\in\Phi}J_{sr}(\phi).
  \end{equation} 


\subsection{Visualization and sensitivity analysis}
To improve interpretability of the results, the sensitivity of the finite-gain stability index (and tracking performance) to key design parameters can be analyzed throug parametric analysis.
Specifically, surface or contour plots of $L(\phi)$ and $E(\phi)$ are generated over a two-dimensional grid defined by the prediction horizon $T_p$ and the ratio $\kappa = \mathrm{Tr}(Q)/\mathrm{Tr}(R)$. These plots show how variations in $T_p$ and in the relative weighting between states and inputs influence the closed-loop stability margin (and tracking accuracy).


\subsection{Summary of the design algorithm}
Algorithm~\ref{alg:design} summarizes the proposed procedure.
\begin{algorithm}[htbp]
\caption{Selection of the optimal NMPC configuration via finite-gain analysis}
\label{alg:design}

\textbf{Input:} System \eqref{eq:plant}, $\mathcal{X}_0$, $\mathcal{R}$, $x_{max}$, $u_{max}$

\textbf{Output:} $\phi^\star$

\begin{algorithmic}[1]

  \State Choose nominal $\phi_{\mathrm{nom}}$ and compute minimal $\tau^\star$ satisfying \eqref{eq:tau_choice}.
  \State Construct the NMPC configuration set $\Phi$ and the scenario set $\mathcal{S}$.
  \ForAll{$\phi\in \Phi$}:
  \ForAll{$s^i\in\mathcal{S}$}:
      \State Simulate closed-loop for $t=1,\dots,\tau^\star$.
      \State Compute $E(\phi,s^i)$ and $F^{\tau^\star}_t(\phi,s^i)$.
  \EndFor
    \State Compute $E(\phi)$ and $L(\phi)$.
    \EndFor
  \State Select $\phi^\star$ through Eq.~\eqref{eq:Jc}.
  \State Produce surface plots and, if necessary, refine the candidate grid.
\end{algorithmic}
\end{algorithm}

By exploiting the finite-gain stability condition of Theorem~\ref{th:fgs_dist}, the proposed procedure provides a systematic and computationally efficient method for obtaining an optimal NMPC configuration through a Monte Carlo campaign in which each closed-loop simulation is performed only over the horizon $\tau^*$. This significantly reduces the computational effort compared to traditional long-horizon simulations that run until the system reaches the reference target.

==> old_intro.tex <==
In the framework of optimal control, Model Predictive Control (MPC) has emerged -- in the recent decades -- as one of the most effective and reliable control methodologies. Its success stems from its inherent ability to provide optimal control commands for multi-variable systems in the presence of inputs, outputs, and state constraints handling constrained control problems in both linear and nonlinear settings \cite{rawlings2017}.

One of the main MPC features is the prediction of the system's behavior along a finite-time horizon. Nevertheless, most of the time a simplified and/or approximated model of the plant is employed, when the latter is highly complex and/or not completely known, especially for those applications where a low computational burden of the algorithm, for \emph{fast} controller application, is required \cite{BOGGIO2023}. 

In these situations, non-accurate predictions due to modeling errors or neglected disturbances may seriously hamper the controller's performance, pauperizing the stability properties of the closed-loop. Indeed, while nowadays the MPC nominal stability is well established (see, e.g. \cite{rawlings2017,Mayne2013}, and the reference therein) both in linear and nonlinear frameworks, the analysis of its intrinsic stability under uncertainties/disturbances remains an attractive topic of research, particularly in highlighting the differences between the classical Lyapunov arguments and the alternative finite gain stability (FGS) (see, e.g., \cite{book-khalil-2002, hill1980}) and input-to-state stability concepts \cite{Limon2009}.

An exhaustive discussion on Lyapunov stability in presence of external disturbances is proposed in the recent monograph by \cite{rawlings2017}, based on the early works \cite{teel2004, kellet2004}. In the referenced work, the closed-loop in proved to be stable under reasonable bounds of the uncertainty, as for the unperturbed case, by a suitable selection of the controller's terminal ingredients, i.e., a terminal cost and its associated local terminal controller, and a control admissible forward invariant terminal set to be employed as terminal constraint. 
Nevertheless, the Lyapunov-based approach does not provide any specific guideline for defining disturbance bounds, hindering the chances to define a constructive framework for stabilizing MPC design, not explicitly quantifying how bounded disturbances affect closed-loop performance.
%, a limitation in applications where robustness and performance degradation need to be explicitly characterized in order to quantify the robustness margin of the controller. 

In this context, FGS \cite{book-khalil-2002, ZACCARIAN2003} offers a more flexible and practically meaningful concept of stability. Indeed, instead of requiring a Lyapunov function descent property, finite-gain conditions are able to quantify the sensitivity of the closed-loop system with respect to disturbances through an input–state (or output) relationship, bounding the state tracking error as a function of the disturbance magnitude. 
Importantly, verifying FGS often requires weaker assumptions than constructing a Lyapunov function. Hence, FGS is particularly advantageous for studying the closed-loop stability of the nonlinear MPC (NMPC) controller discussed in this paper.

Usually, the Lyapunov-bases approach suffers -- under peculiar conditions -- from two main drawbacks: i) increased computational complexity arising from the terminal equality/inequality constraint, and ii) limited flexibility in handling pointwise time-varying reference trajectories.
In the former case, if the reference equilibrium pair is strictly feasible, the final constraint can be described by means of a finite number of linear inequalities \cite{Gilbert:Tan:1991:Admissible}. However, the number of linear constraints required can be very large, even for relatively small systems \cite{Kerrigan:00}.
On the other hand, the latter drawback remains one of the most challenging issues in the current NMPC framework. Specifically, in Lyapunov-based stabilizing NMPC formulations, the terminal ingredients are typically derived by linearization of the nonlinear system around the desired equilibrium to track (see, e.g., \cite{lazar2018, WAN2003, WAN2003_2, limon2018}). This poses an exceptional challenge when the prescribed reference is likely to change at each sampling instant. In contrast, the FGS framework alleviates these challenges, as it does not require the explicit computation of terminal ingredients to assess the closed-loop stability certificates. Consequently, FGS bears the hallmarks of i) simplified controller design and implementation, and ii) reduced computational burden in solving the associated optimal control problem.

In this paper, we develop a comprehensive finite-gain stability analysis framework for NMPC in the presence of bounded additive disturbances, not accounted in the prediction model. The case where the model is approximated, is a topic of ongoing research. In this context, we derive sufficient conditions under which, given a prescribed reference (potentially time-varying), 
if the initial state is confined within a suitable set of feasible initial conditions, the resulting closed-loop trajectory is asymptotically steered towards the reference. Particularly, by leveraging the concept of stability for linear-time variant (LTV) systems, we quantify the bounds on tracking error in terms of disturbances, with relaxed assumptions on the nonlinear system under investigation.

More importantly, the FGS approach paves to road for proposing the main contribution of the paper: a systematic methodology for selecting a suitable NMPC configuration with FGS guarantees, while providing satisfactory tracking performances. Importantly, in our formulation, we do not need neither to define a local terminal controller nor to impose a terminal constraint to the optimization problem.
The proposed designed procedure follows an offline three-step procedure consisting of i) the determination of the NMPC parameters ensuring the finite-gaom closed-loop stability, ii) a Monte Carlo campaign for trading-off different candidate NMPC configurations and closed-loop data and iii) the selection of the best NMPC by means of suitable evaluation criteria depicting both the stability and the tracking performance behavior of the closed-loop. 

Finally, the effectiveness of the proposed finite-gain stable NMPC is verified by numerical experiments. As test cases, we employ the standard dynamic single-track model representing the lateral and longitudinal nonlinear dynamics of a road vehicles involved in two different road scenarios.
%a twofold scenario: i) a lane keeping application where the vehicle is asked to follow a sinusoidal path depicting a curvilinear urban road and ii) an obstacle-avoidance maneuver for assessing the NMPC capability of ensuring a collision-free operation while preserving stability and maintaining acceptable tracking accuracy after the avoidance phase. 

%\subsection{Outline}
%In Section \ref{sec:nmpc}, we present the general discrete-time NMPC formulation. The finite-gain stability of the closed-loop and its theoretical derivation is depicted in Section \ref{sec:fgs_exact}. In Section \ref{sec:nmpc_des}, we present the systematic methodology for the selection of a suitable NMPC simulations, while the simulated test cases is shown in Section \ref{sec:results}. Finally, conclusions and future lines of research are drawn in Section \ref{sec:conclusion}.
